Beyond the Standard Model Physics at the HL-LHC and HE-LHC

This is the third out of five chapters of the final report [1] of the Workshop on Physics at HL-LHC, and perspectives on HE-LHC [2]. It is devoted to the study of the potential, in the search for Beyond the Standard Model (BSM) physics, of the High Luminosity (HL) phase of the LHC, defined as $3~\mathrm{ab}^{-1}$ of data taken at a centre-of-mass energy of $14~\mathrm{TeV}$, and of a possible future upgrade, the High Energy (HE) LHC, defined as $15~\mathrm{ab}^{-1}$ of data at a centre-of-mass energy of $27~\mathrm{TeV}$. We consider a large variety of new physics models, both in a simplified model fashion and in a more model-dependent one. A long list of contributions from the theory and experimental (ATLAS, CMS, LHCb) communities have been collected and merged together to give a complete, wide, and consistent view of future prospects for BSM physics at the considered colliders. On top of the usual standard candles, such as supersymmetric simplified models and resonances, considered for the evaluation of future collider potentials, this report contains results on dark matter and dark sectors, long lived particles, leptoquarks, sterile neutrinos, axion-like particles, heavy scalars, vector-like quarks, and more. Particular attention is placed, especially in the study of the HL-LHC prospects, to the detector upgrades, the assessment of the future systematic uncertainties, and new experimental techniques. The general conclusion is that the HL-LHC, on top of allowing to extend the present LHC mass and coupling reach by $20-50\%$ on most new physics scenarios, will also be able to constrain, and potentially discover, new physics that is presently unconstrained. Moreover, compared to the HL-LHC, the reach in most observables will generally more than double at the HE-LHC, which may represent a good candidate future facility for a final test of TeV-scale new physics.

==> section2SUSY/sub21_5.tex <==
\subsubsection{\cmsC{Electroweak production of a top squark and the lightest chargino}}

\contributors{A. Kalogeropoulos, D. Marlow, CMS}

\newcommand{\cone}{\PSGcpmDo}
\providecommand{\none}{\ensuremath{\widetilde{\chi}^{0}_{1}}\xspace} 
\newcommand{\mumu}{\ensuremath{\mu\mu}\xspace}
\newcommand{\me}{\ensuremath{e\mu}\xspace}
\newcommand{\ee}{\ensuremath{ee}\xspace}
\newcommand{\irel}{\ensuremath{I_{\text{rel}}}\xspace}
\newcommand{\dR}{\ensuremath{\Delta R}\xspace}
\newcommand{\MT}{\ensuremath{M_{\text{T}}}\xspace}
\newcommand{\tjets}{\ensuremath{t\bar{t}}\text{+jets}\xspace}
\newcommand{\MTdil}{\ensuremath{M_{\text{T}}(\ell\ell)}\xspace}
\newcommand{\wjets}{\ensuremath{\PW}+jets\xspace}
\newcommand{\zjets}{\ensuremath{\Z}+jets\xspace}
\newcommand{\njet}{\ensuremath{N_{\text{jet}}}\xspace}
\newcommand{\ntag}{\ensuremath{N_{\text{tag}}}\xspace}
\newcommand{\nj}{\ensuremath{N_{\text{jet}}}\xspace}



In the context of the MSSM, the associated pair production of the \PSQtDo and the \cone via an EWK process may occur at the LHC. The EWK production cross sections of coloured SUSY particles can be orders of magnitude smaller than strong production, and thus are less well constrained. The unprecedented dataset expected at the HL-LHC provides a unique opportunity to probe such rare processes. 
While the discovery and exclusion potential of strong production of \PSQtDo\ at the HL-LHC is greater,  EWK \PSQtDo-\cone\ production can provide important complementary information by further probing the compressed phase space. In particular, in the event of a discovery, EWK \PSQtDo-\cone\ production can help in determining the mixing angle tan-$\beta$~\cite{Duan:2016vpp,Beccaria:2006wz}, as well as probing the mixing of the two top squark flavour eigenstates ($\tilde{t}_L$ and $\tilde{t}_R$)~\cite{Duan:2016vpp}.

This analysis investigates the EWK pair production of the hypothetical \PSQtDo\ and the lightest \cone~\cite{CMS-PAS-FTR-18-039}. Two scenarios are considered: the \PSQtDo\ is mass degenerate with the \cone; or $m_{\PSQtDo}= 2 \times m_{\cone}$ and the \none\ is wino-like and thus almost degenerate in mass with the \cone, with $m_{\cone} - m_{\none} = 20 \GeV$, henceforth mentioned as the ``compressed model.'' The signal cross sections have been computed  at NLO with \texttt{MadGolem}~\cite{Goncalves:2014axa,GoncalvesNetto:2012nt,Binoth:2011xi} using the \texttt{CTEQ6.1} PDF set~\cite{Stump:2003yu}. The production cross sections for the compressed models are higher than the mass degenerate models by approximately a factor of two. In both scenarios, the \PSQtDo\ is assumed to decay to a top quark and the \none, whereas the \cone\ decays to a \PW\ boson and a \none. Figure~\ref{fig:sms} shows a diagram of the production and decay of the \PSQtDo-\cone\ pair.

\begin{figure}[t]
\begin{center}
\includegraphics[width=0.3\textwidth]{\main/section2SUSY/img/TStopChi}
\caption{Diagram of the electroweak production of \PSQtDo-\cone\ pairs.
\label{fig:sms}}
\end{center}
\end{figure}

%\begin{figure}[t]
%\centering
%\begin{minipage}[t][\minipageheightdp][t]{\minipagewidthdp}
%\centering
%\includegraphics[width=\figuremaxwidthdp,height=\figuremaxheightdp,keepaspectratio]{\main/section2SUSY/img/TStopChi}
%\end{minipage}
%\caption{Diagram of the electroweak production of \PSQtDo-\cone\ pairs.
%\label{fig:sms}}
%\end{figure}

Selected events contain exactly two isolated oppositely charged lepton candidates, muons or electrons, of the same (SF) or opposite-flavour (OF) forming three categories of dileptonic final states: \mumu, \ee, and \me. In the SF case, the leptons are required to have a transverse momentum $\pt > 30 \GeV$ and pseudorapidity $|\eta| <  2.4$ (1.6) for muons (electrons), whereas in the case of OF leptons, the leading (trailing) lepton is required to have $\pt > 25$ $(15) \GeV$. No more than four jets with $\pt>20\GeV$ and $|\eta|<2.4$, separated from the leptons using a cone of  \dR $>0.5$, are allowed. In order to suppress the dominant \tjets background, up to one candidate \PQb tagged jet (\ntag) is allowed. Tagged \PQb jets are identified with the medium working point of the DeepCSV \PQb tagging algorithm~\cite{Sirunyan:2017ezt}, with an efficiency of 68\%, while the misidentification rates for jets originating from charm quarks or light-flavour quarks and gluons are approximately 12 and 1.1\%, respectively.

The invariant mass of the dilepton system $M_{\ell\ell}$ is required to be $75 < M_{\ell\ell} < 105\GeV$ ($50 < M_{\ell\ell} < 80\GeV$) for the SF (OF) channels. Low-mass resonances are rejected with a $M_{\ell\ell} > 20\GeV$ cut, and the requirement $\dR\ < 3.0$ between the two leptons is imposed. A cut on the missing transverse momentum $\met > 80\GeV$ effectively rejects 99\% (60\%) of the remaining \zjets (\tjets) background. 

A cut on the transverse mass (\MT) defined as $\MT(\ell, \met)^2 \equiv  2 \pt^{\ell} \met (1 - \cos \Delta\phi(\ell, \met))$, which presents a characteristic kinematic feature in the form of an endpoint at the mass of the mother particle, of $\MT>80\GeV$ is imposed for all channels and for each of selected leptons in the final state. After applying the baseline selection, \tjets is the dominant background, contributing approximately 75\% of the total background, followed by single top quark production that contributes approximately 12\%. Additional contributions from \wjets, diboson, triboson, and the associated production of a vector boson and $t\bar{t}$ (henceforth collectively labelled as "Other SM") and \zjets are 8-10\% and 1-6\%, depending on the final state. 

A variation of the \MT is considered in this search, when the $\vec{\pt}$ of the leptons are first vectorially summed before being used to determine the 
$\MTdil = \MT$(
$\vec{\ell}, 
\vec{E}
_{\rm{T}}
^{\textrm{miss}}$
), where
$\vec{\ell}=\vec{\ell_1}+\vec{\ell_2}$.
The signal regions are defined following the categorisation of events according to the number of \ntag, zero or one, as well as $\met$ and \MTdil, as summarised in~\tabb{tab:SR}. In total, 14 search regions are considered for each of the three dilepton final states.


\begin{table}[t]
\begin{center}
\small{\begin{tabular}{cc}
\hline
\hline
$\met$ (GeV)          & \MTdil (GeV)   \\ 
\hline \hline
 < 200   &  {[}100-150{]}, {[}150-200{]}, > 200  \\ 
 \hline
{[}200-300{]}    & {[}100-300{]},  > 300  \\  
\hline
> 300 &  {[}100-300{]},  > 300    \\ 
\hline \hline
\end{tabular}
\caption{Definition of the signal-enriched search region bins, where each bin is further divided into $\ntag=0$ and $\ntag=1$.
\label{tab:SR}}}
\end{center}
\end{table}


The dominant experimental uncertainties are those originating from the modelling of the jet energy scale and resolution, 
from the lepton efficiency, the \PQb tagging efficiency, and the integrated luminosity. These uncertainties are correlated among the background processes and the signal yields. For all backgrounds, a 5\% normalisation uncertainty is considered, which is consistent with the treatment of the dominant \tjets background for related searches by the CMS Collaboration~\cite{CERN-EP-2018-312,Sirunyan:2018vig}. The same 5\% uncertainty is also applied to the signal normalisation, which is conservative compared to the 1\% or less uncertainty that \texttt{MadGolem} provides. The simulation modelling of the $\met$ and \MTdil variables is assumed to be adequate, based on recent results from a similar search performed by the CMS Collaboration~\cite{CERN-EP-2018-312}.

Figure~\ref{res:mm} shows the expected event yields from SM background processes for all  of the search regions and the three dilepton final states. Four benchmark signal model points are overlaid, where SA corresponds to $m_{\PSQtDo}=m_{\cone} = 175 \GeV, m_{\none} = 1\GeV$, SB corresponds to  $m_{\PSQtDo}= 2\times m_{\cone} = 87.5 \GeV, m_{\none} = 67.5\GeV$,  SC corresponds to $ m_{\PSQtDo}=m_{\cone} = 200 \GeV, m_{\none} = 25\GeV$, and SD corresponds to $m_{\PSQtDo}= 2\times m_{\cone} = 125 \GeV, m_{\none} = 105\GeV$. Models SA and SC have a mass-degenerate \PSQtDo and \cone system, and a low-mass \none, while SB and SD are characterised by a \cone-\none system that is nearly mass degenerate.

The results are interpreted with the use of simplified models. Expected upper limits on the production cross section at the 95\% confidence level (CL) are calculated using the asymptotic formulae~\cite{Cowan:2010js} of the CLs criterion~\cite{Junk:1999kv,Read:2002hq}. The upper limits are shown in~\fig{res:modelA_LSP1} for a mass-degenerate \PSQtDo\-\cone\ system and for $m_{\none} = 1, 25$, and $50\GeV$. Table~\ref{tab:res_modelB} summarises the ratio of the experimental upper limits on the production cross sections and the theoretical value for models with $m_{\cone} = 2\times m_{\cone}$ and $m_{\cone}-m_{\none} = 20\GeV$. 

\begin{figure*}[t]
\centering
\begin{minipage}[t][\minipageheighttp][t]{\minipagewidthtp}
\centering
\includegraphics[width=\figuremaxwidthtp-3mm,height=\figuremaxheighttp,keepaspectratio]{\main/section2SUSY/img/met_MTDil6_10_Merged5_noJets_3000_MuMu.pdf}
\end{minipage}
\begin{minipage}[t][\minipageheighttp][t]{\minipagewidthtp}
\centering
\includegraphics[width=\figuremaxwidthtp-3mm,height=\figuremaxheighttp,keepaspectratio]{\main/section2SUSY/img/met_MTDil6_10_Merged5_noJets_3000_ElEl.pdf}
\end{minipage}
\begin{minipage}[t][\minipageheighttp][t]{\minipagewidthtp}
\centering
\includegraphics[width=\figuremaxwidthtp-3mm,height=\figuremaxheighttp,keepaspectratio]{\main/section2SUSY/img/met_MTDil6_10_Merged5_noJets_3000_MuEl.pdf}
\end{minipage}
\caption{\label{res:mm}Expected event yields from benchmark signal models and SM background processes in the 14 search regions for the \mumu (left), \ee\ (middle), and \me (right) final states.}
\end{figure*}

%\begin{figure}[t]
%\centering
%\begin{minipage}[t][\minipageheightdp][t]{\minipagewidthdp}
%\centering
%\includegraphics[width=\figuremaxwidthdp,height=\figuremaxheightdp,keepaspectratio]{\main/section2SUSY/img/met_MTDil6_10_Merged5_noJets_3000_MuMu.pdf}
%\end{minipage}
%\begin{minipage}[t][\minipageheightdp][t]{\minipagewidthdp}
%\includegraphics[width=\figuremaxwidthdp,height=\figuremaxheightdp,keepaspectratio]{\main/section2SUSY/img/met_MTDil6_10_Merged5_noJets_3000_ElEl.pdf}
%\end{minipage}
%\begin{minipage}[t][\minipageheightdp][t]{\minipagewidthdp}
%\includegraphics[width=\figuremaxwidthdp,height=\figuremaxheightdp,keepaspectratio]{\main/section2SUSY/img/met_MTDil6_10_Merged5_noJets_3000_MuEl.pdf}
%\end{minipage}
%\caption{\label{res:mm}Expected event yields from benchmark signal models and SM background processes in the 14 search regions for the \mumu (left), \ee\ (middle), and \me (right) final states.}
%\end{figure}

\begin{figure*}[t]
\centering
\begin{minipage}[t][\minipageheighttp][t]{\minipagewidthtp}
\centering
\includegraphics[width=\figuremaxwidthtp-3mm,height=\figuremaxheighttp,keepaspectratio]{\main/section2SUSY/img/single-stop14TeV_1Dexclusion_1GeV_met_MTDil6_10Brazil_Merged5I_noJets_3000invfb.pdf}
\end{minipage}
\begin{minipage}[t][\minipageheighttp][t]{\minipagewidthtp}
\centering
\includegraphics[width=\figuremaxwidthtp-3mm,height=\figuremaxheighttp,keepaspectratio]{\main/section2SUSY/img/single-stop14TeV_1Dexclusion_25GeV_met_MTDil6_10Brazil_Merged5I_noJets_3000invfb.pdf}
\end{minipage}
\begin{minipage}[t][\minipageheighttp][t]{\minipagewidthtp}
\centering
\includegraphics[width=\figuremaxwidthtp-3mm,height=\figuremaxheighttp,keepaspectratio]{\main/section2SUSY/img/single-stop14TeV_1Dexclusion_50GeV_met_MTDil6_10Brazil_Merged5I_noJets_3000invfb.pdf}
\end{minipage}
\caption{\label{res:modelA_LSP1}Upper limits on the production cross section for a mass-degenerate \PSQtDo-\cone\ system and for $m_{\none} = 1,25\rm{~and~}50\GeV$ (left, middle and right, respectively).}
\end{figure*}

%\begin{figure}[t!b]
%\centering
%\begin{minipage}[t][\minipageheightdp][t]{\minipagewidthdp}
%\centering
%\includegraphics[width=\figuremaxwidthdp,height=\figuremaxheightdp,keepaspectratio]{\main/section2SUSY/img/single-stop14TeV_1Dexclusion_1GeV_met_MTDil6_10Brazil_Merged5I_noJets_3000invfb.pdf}
%\end{minipage}
%\begin{minipage}[t][\minipageheightdp][t]{\minipagewidthdp}
%\includegraphics[width=\figuremaxwidthdp,height=\figuremaxheightdp,keepaspectratio]{\main/section2SUSY/img/single-stop14TeV_1Dexclusion_25GeV_met_MTDil6_10Brazil_Merged5I_noJets_3000invfb.pdf}
%\end{minipage}
%\begin{minipage}[t][\minipageheightdp][t]{\minipagewidthdp}
%\includegraphics[width=\figuremaxwidthdp,height=\figuremaxheightdp,keepaspectratio]{\main/section2SUSY/img/single-stop14TeV_1Dexclusion_50GeV_met_MTDil6_10Brazil_Merged5I_noJets_3000invfb.pdf}
%\end{minipage}
%\caption{\label{res:modelA_LSP1}Upper limits on the production cross section for a mass-degenerate \PSQtDo-\cone\ system and for $m_{\none} = 1,25\rm{~and~}50\GeV$ (left, middle and right, respectively).}
%\end{figure}


\begin{table}[!h]
\begin{center}
\small{\begin{tabular}{ccccccc}
\hline
$m_{\PSQtDo}$  (\GeV) & $m_{\none}$  (\GeV) & $-2\sigma$ &  $-1\sigma$ & expected & $+1\sigma$   & $+2\sigma$ 
\\ \hline
175 &   67.5 & 0.82 &  1.10 &  1.53  &  2.13 &  2.85  \\ \hline
200 &   80 & 0.61 &  0.81 &  1.13  &  1.57 &  2.11  \\ \hline
225 &   92.5 &1.27 &  1.69 &  2.36  &  3.28 &  4.39  \\ \hline
250 &   105 & 1.04 &  1.38 &  1.92  &  2.68 &  3.58  \\ \hline
300 &  130 &  1.25 &  1.66 &  2.31  &  3.23 &  4.34  \\ \hline 
\end{tabular}
\caption{Ratio of the experimental upper limits on the production cross sections and the theoretical value for models with $m_{\PSQtDo} = 2 \times m_{\cone}$ and $m_{\cone}-m_{\none}= 20\GeV$. Changes to the expected value under $\pm1$ and $\pm2$ variations in systematic uncertainties are also provided.
\label{tab:res_modelB}}}
\end{center}
\end{table}

For the mass degenerate scenario, \PSQtDo\ masses up to approximately 300\GeV are expected to be excluded when $m_{\none}$ is less than 50 GeV. For the compressed scenarios, the upper limit on the production cross section for $m_{\PSQtDo} = 175\GeV$ is approximately a factor 1.5 times the theoretical value.
